Latent Graph Inference using Product Manifolds

Graph Neural Networks usually rely on the assumption that the graph topology is available to the network as well as optimal for the downstream task. Latent graph inference allows models to dynamically learn the intrinsic graph structure of problems where the connectivity patterns of data may not be directly accessible. In this work, we generalize the discrete Differentiable Graph Module (dDGM) for latent graph learning. The original dDGM architecture used the Euclidean plane to encode latent features based on which the latent graphs were generated. By incorporating Riemannian geometry into the model and generating more complex embedding spaces, we can improve the performance of the latent graph inference system. In particular, we propose a computationally tractable approach to produce product manifolds of constant curvature model spaces that can encode latent features of varying structure. The latent representations mapped onto the inferred product manifold are used to compute richer similarity measures that are leveraged by the latent graph learning model to obtain optimized latent graphs. Moreover, the curvature of the product manifold is learned during training alongside the rest of the network parameters and based on the downstream task, rather than it being a static embedding space. Our novel approach is tested on a wide range of datasets, and outperforms the original dDGM model.

==> tables/homophilic_extra2.tex <==

\begin{table*}[htbp!]
    \centering
    \caption[Results for classical homophilic datasets combining GCN diffusion layers with the dDGM latent graph inference system and using single model spaces to construct the latent graphs. The dDGM uses the original dataset graph as inductive bias. Different $k$ values for the Gumbel Top-k trick are applied.]{Results for classical homophilic datasets combining GCN diffusion layers with the dDGM latent graph inference system and using single model spaces to construct the latent graphs. The dDGM uses the original dataset graph as inductive bias. Different $k$ values for the Gumbel Top-k trick are applied. Here, the GCN model, which leverages the dataset graph connectivity structure, is used as baseline.
    }
    
\scalebox{0.72}{
    \begin{tabular}{l cccccc}
    \toprule 
         &
         &
         \textbf{Cora} &  
         \textbf{CiteSeer} & 
         \textbf{PubMed} &
         \textbf{Physics} &
         \textbf{CS}
         \\
         
         Homophily level &
         &
         0.81 &
         0.74 &
         0.80 &
         0.93&
         0.80
         
          \\ 
         
         Nodes &
        &
         2,708 &
         3,327 &
         18,717 &
          34,493 &
          18,333
          \\
          
        Features &
        &
         1,433 &
         3,703 &
         500 &
          8,415 &
          6,805
          \\
         
         Edges &
        &
        5,278 &
         4,676 &
         44,327 &
         247,962 &
         81,894
          \\
         
         Classes &
        &
        7 &
         6 &
         3 &
         5 &
         15 \\
         
         Average Degree & 
        &
        3.9 &
         2.77 &
         4.5 &
         14.38 &
         8.93
         
          
         
         \\ 
         \midrule
         
         Model & $k$ &
         \multicolumn{5}{c}{Accuracy $(\%)$ $\pm$ Standard Deviation}
         
         \\
          \midrule
         GCN-dDGM-E & 3&
         $ 80.44 {\scriptstyle \pm 4.60 }$ &
         $ 70.18 {\scriptstyle \pm 1.46}$ &
         $ 87.45 {\scriptstyle \pm 0.72 }$ & 
         $ \secondd{96.03 {\scriptstyle \pm 0.41}}$ &
         $ 85.98 {\scriptstyle \pm 2.59}$
         \\
         
         GCN-dDGM-H & 3&
         $ 80.31 {\scriptstyle \pm 4.30 }$ &
         $ 69.78 {\scriptstyle \pm 1.56}$ &
         $ 85.79 {\scriptstyle \pm 0.73 }$ & 
         $ 95.29 {\scriptstyle \pm 0.43}$ &
         $ 85.95 {\scriptstyle \pm 2.58}$
         \\
         
         GCN-dDGM-S & 3&
         $ 73.26 {\scriptstyle \pm 4.33}$ &
         $ 67.98 {\scriptstyle \pm 2.21}$ &
         $ 81.39 {\scriptstyle \pm 1.00}$ & 
         $ 91.60 {\scriptstyle \pm 0.55 }$ &
         $ 76.76 {\scriptstyle \pm 4.65}$\\
         
        
         

        
        \midrule
         GCN-dDGM-E& 5&
         $ 82.74 {\scriptstyle \pm 4.42 }$ &
         $ 71.78 {\scriptstyle \pm 1.50}$ &
         $ \thirdd{87.60 {\scriptstyle \pm 0.69}}$ & 
         $ 95.96 {\scriptstyle \pm 0.40}$ &
         $ 87.88 {\scriptstyle \pm 2.55}$\\
         
         GCN-dDGM-H & 5&
         $ 80.80 {\scriptstyle \pm 4.43}$ &
         $ 67.53 {\scriptstyle \pm 2.12}$ &
         $ 87.58 {\scriptstyle \pm 0.71}$ & 
         $ \first{96.06 {\scriptstyle \pm 0.42}}$ &
         $ 87.65 {\scriptstyle \pm 2.56}$\\
         
         GCN-dDGM-S & 5&
         $  80.81{\scriptstyle \pm 2.30}$ &
         $ 71.81{\scriptstyle \pm 1.20}$ &
         $ 77.65{\scriptstyle \pm 1.01}$ & 
         $  95.91{\scriptstyle \pm 0.41 }$ &
         $ 80.73 {\scriptstyle \pm 4.62}$\\
         
         
         
         \midrule
         GCN-dDGM-E & 7&
         $ 82.11 {\scriptstyle \pm 4.24 }$ &
         $ \thirdd{72.35 {\scriptstyle \pm 1.92 }}$ &
         $ \secondd{87.69 {\scriptstyle \pm 0.67 }}$ & 
         $ 95.50 {\scriptstyle \pm 1.25 }$ &
         $ 87.17 {\scriptstyle \pm 3.82 }$\\
         
         GCN-dDGM-H & 7&
         $  \first{84.68 {\scriptstyle \pm 3.31 }}$ &
         $ 70.43 {\scriptstyle \pm 4.95 }$ &
         $ \first{87.74 {\scriptstyle \pm 0.72 }}$ & 
         $  \first{96.06 {\scriptstyle \pm 0.46 }}$ &
         $ \first{88.78 {\scriptstyle \pm 2.24 }}$\\
         
         GCN-dDGM-S & 7&
         $ 80.44 {\scriptstyle \pm 5.26}$ &
         $ \first{72.89 {\scriptstyle \pm 2.00 }}$ &
         $ 87.13 {\scriptstyle \pm 0.66 }$ & 
         $ 95.76 {\scriptstyle \pm 0.43 }$ & 
         $ 84.16 {\scriptstyle \pm 2.78 }$\\
         
      
         
         \midrule
         GCN-dDGM-E & 10&
         $ 81.67 {\scriptstyle \pm 5.74 }$ &
         $ \secondd{72.44 {\scriptstyle \pm 2.81 }}$ &
         $ 85.45 {\scriptstyle \pm 4.32 }$ & 
         $ \thirdd{95.99 {\scriptstyle \pm 0.49 }}$ &
         $ \thirdd{88.19 {\scriptstyle \pm 3.51}}$\\
         
         GCN-dDGM-H & 10&
         $ \secondd{83.15 {\scriptstyle \pm 3.20 }}$ &
         $ 71.54 {\scriptstyle \pm 1.46 }$ &
         $ \secondd{87.69 {\scriptstyle \pm 0.76 }}$ & 
         $ 95.84 {\scriptstyle \pm 0.73}$ &
         $ \secondd{88.49 {\scriptstyle \pm 2.21 }}$\\
         
         GCN-dDGM-S & 10&
         $ 82.70 {\scriptstyle \pm 3.22 }$ &
         $ 72.29 {\scriptstyle \pm 2.87 }$ &
         $ 87.38 {\scriptstyle \pm 0.69 }$ & 
         $  \secondd{96.03 {\scriptstyle \pm 0.44 }}$ & 
         $ 85.20 {\scriptstyle \pm 4.07 }$\\
         
        
         
         \midrule
         GCN & N/A &
         $ \thirdd{83.11 {\scriptstyle \pm 2.29}}$ &
         $ 69.97 {\scriptstyle \pm 2.06}$ &
         $ 85.75 {\scriptstyle \pm 1.01}$ & 
         $ 95.51 {\scriptstyle \pm 0.34}$ &
         $ 87.28 {\scriptstyle \pm 1.54 }$\\ 
         

         
         \bottomrule
         
    \end{tabular}}
    
    \label{tab:homophilic_extra2}
\end{table*}
